Robust and Precision Satellite Formation Flying Guidance Using Adaptive Optimal Control Techniques

The main focus of the work presented in this thesis is to develop an optimal control based formation flying control strategy for high precision formation flying of small satellites that have restricted computation and storage capacity. Using the recently developed model predictive static programming (MPSP), and Generalized MPSP algorithm a suboptimal guidance logic is presented for the formation flying of small satellites. The proposed guidance scheme is valid both for high eccentricity chief satellite orbits as well as the large separation distance between the chief and deputy satellites. Comparative study with standard Linear Quadratic Regulator (LQR) solution (which serves as a guess solution for MPSP) and another nonlinear controller, Finite-time State-Dependent Ricatti Equation (SDRE) reveals that MPSP guidance achieves the objective with higher accuracy and with a lesser amount of control usage.

==> Copyright.tex <==

\newpage
\ \ \ \ \ \ \

\thispagestyle{empty}\setcounter{page}{0}

\vspace{3in}
\begin{center}
{\Large\bf \copyright Girish Joshi \\ \vspace{0.2in} June 2013 \\ \vspace{0.2in} All rights reserved}
\end{center}
\newpage
\ \ \ \ \ \ \

\thispagestyle{empty}\setcounter{page}{0} 

==> Postscript/pubs.tex <==
\begingroup

\leftskip=-1.5in



\ChapterStar{Publications from this thesis}
\addcontentsline{toc}{chapter}{\hspace*{-1.2in}Publications from this thesis}%
{\advance \leftskip0.8in \noindent

\begin{list}{}{\leftmargin=-0.7in}

\item[1.] Manathara, J. G., \&
Ghose, D. (2011). A reactive algorithm for collision avoidance among
multiple unmanned aerial vehicles. (manuscript under preparation).

\item[2.] Manathara, J. G., \&
Ghose, D. (2011). Multiple UAV collision avoidance using realistic
UAV models. {\em Journal of Aircraft Engineering and Aerospace
Technology}. (under revision).

\item[3.] Manathara, J. G., \&
Ghose, D. (2011). Rendezvous of multiple UAVs under collision
avoidance using consensus. {\em Journal of Aerospace Engineering}.
(under revision).

\item[4.]  Manathara, J. G., Sujit, P. B., \& Beard, R. W. (2011). Multiple UAV
coalitions for a search and prosecute mission. {\em Journal of
Intelligent and Robotic Systems,} 62, pp.~125--158. DOI:
10.1007/\penalty 0 s10846-010-9439-2

\item[5.] George, J., \& Ghose, D. (2010). Multiple UAV collision avoidance using
realistic UAV models. In {\em Proceedings of the International
Conference on Intelligent Unmanned Systems,} Bali, Indonesia.

\item[6.] George, J., \& Ghose, D. (2010). Multiple UAV rendezvous under collision
avoidance. In {\em Proceedings of the International Conference on
Intelligent Unmanned Systems,} Bali, Indonesia.

\item[7.] George, J. M., Sujit, P. B., \& Sousa, J. B. (2010). Coalition formation
with communication delays and maneuvering targets. In {\em AIAA
Guidance, Navigation and Control Conference and Exhibit,} Toronto,
Canada. Paper No.~AIAA-2010-8422.

\item[8.] George, J. M., Sujit, P. B., Sousa, J. B., \& Pereira, F.
L. (2010). Coalition formation with communication ranges and moving
targets. In {\em Proceedings of the American Control Conference,}
Baltimore, USA, pp. 1605--1610.

\item[9.] George, J. M., Pinto, J., Sujit, P. B., \& Sousa, J. B. (2010). Multiple
UAV coalition formation strategies. In {\em Proceedings of 9th
International Conference on Autonomous Agents and Multiagent Systems
(AAMAS 2010),} Toronto, Canada, pp. 1503--1504.

\item[10.] George, J., \& Ghose, D. (2009). A reactive inverse PN algorithm for
collision avoidance among multiple unmanned aerial vehicles. In {\em
Proceedings of the American Control Conference,} Missouri, USA, pp.
3890--3895.

\item[11.] George, J., \& Ghose, D. (2009). A 3-D reactive algorithm for collision
avoidance among multiple unmanned aerial vehicles in dense traffic
situations. In {\em Proceedings of the International Conference and
Exhibition on Aerospace Engineering,} Bangalore, India, pp.
1215--1222.

\end{list}}

\endgroup


==> Preamble/abstract.tex <==
%=============================================================================
%=====================Abstract===============================================
%============================================================================


\ChapterStar{Abstract}
\addcontentsline{toc}{chapter}{\hspace*{-1.2in}Abstract\vspace*{-3.5mm}}%
{\advance\leftskip0.8in \noindent 
\textbf{T}his report studies the collective motion of \textit{\textbf{all-to-all heterogeneously coupled}} self-propelled particles moving at unit speed. Two states of collective motion: \textbf{\textit{synchronized state}} and \textbf{\textit{balanced state}} are primarily described. The synchronized state implies that, at all times, all of the particles have the same direction of motion. On the other hand, collective motion with balanced state has a fixed center of mass. For example, when two particles head in opposite directions, their center of mass always stays at rest.

At first, this report addresses the problem of stabilization of \textbf{\textit{parallel}} and \textbf{\textit{circular formations}} of a group of particles. Parallel formation is characterized by a common orientation for all the particles with arbitrary relative spacing, and circular formation is characterized by a common circular orbit of the particles around a fixed point. To attain these formations, each particle adapts its orientation, that is, the direction of its unit velocity vector according to some decentralized control algorithms. These control algorithms operate with heterogeneous gains and are derived by assuming an analogy between the particle model and the phase model of coupled oscillators. According to this analogy, the velocity vector of each particle can be represented as the phase of the oscillator. The control law is separated into two parts as \textbf{\textit{orientation control}} that controls the relative orientation of the particles, and \textbf{\textit{spacing control}} that controls their relative spacing.

Finally, this thesis discusses the consequences of selecting \textit{\textbf{heterogeneous controller gains}}. Most of the existing literature studies collective motion of multiple agents when they are coupled through homogeneous gains. This type of homogeneous coupling among agents has limited applications in the field of aerial and underwater vehicles. As an extension, we have assumed that the particles are heterogeneously coupled, and that the controller gains can be deterministically varied. This assumption opens some interesting possibilities regarding the formation. For example, we can propagate the formation to the desired location by a proper tuning of these heterogeneous gains. In this context, some analytical results regarding the position of convergence point and the final velocity directions of particles, are discussed.


In summary, this report contributes a special kind of cooperative control framework for the heterogeneously coupled particles which facilitates the formation to relocate at any desired position by the proper selection of the heterogeneous controller gains.




}


==> Preamble/ack.tex <==
\ChapterStar{Acknowledgements}
\addcontentsline{toc}{chapter}{\hspace*{-1.2in}Acknowledgements\vspace*{-3.5mm}}%
{\advance\leftskip0.8in \noindent I express my deep sense of gratitude to my research advisor \textbf{Prof. Debasish Ghose} for his able guidance and useful suggestions, which helped me in completing the project work, on time. I am much indebted to him for his encouragement and patience whenever I found myself hands-up. I feel proud to memorize his continuous effort that he devoted to correct my report when he was out of station.

I take immense pleasure in thanking Shashi Ranjan Kumar, Joel Jeorge and Kaushik Das for their continuous support and help.

Finally, yet importantly, I would like to thank Almighty God Whose invincible power has guided me to complete this report.

}


==> Preamble/notations.tex <==
%----------------------------------------------------------------------

%                    Notations


%------------------------------------------------------------------

\ChapterStar{Notations}

\addcontentsline{toc}{chapter}{\hspace*{-1.2in}Notations}

{\advance\leftskip0.8in \noindent
%A list of notations frequently used in the thesis is given below.

\begin{tabular}{lp{5.0in}}
%%$\mathbb{R}$                   &  The set (field) of real numbers\\ \\
%%\begin{tabbing}
%%\=firstcolumnlength \=  secondcolumnlength \\
\textbf{$r_k$} & Position of $k$-th particle\\ \\
\textbf{$V_k$} & Velocity of $k$-th particle\\ \\
$\theta_k$ & Velocity direction of $k$-th particle\\ \\
$\omega_0$ & Angular frequency of particles\\ \\
$u_k$ & Control input for $k$-th particle\\ \\
$K_k$ & Controller gain for $k$-th particle\\ \\
$q_k$ & Controller gain for $k$-th particle in circular formation\\ \\
$Q_k$ & Controller gain for $k$-th particle in synchronized and balanced circular formation\\ \\
$c_k$ & Center of the circle traversed by $k$-th particle\\ \\
$r$ & Modulus of order parameter\\ \\
$\psi$ & Average phase of oscillators\\ \\
$\omega_k$ & Natural frequency of $k$-th oscillator\\ \\
$u^\textrm{{ori}}$ & Orientation control\\ \\
$u^\textrm{{spac}}$ & Spacing control\\ \\
$U$ & Orientation potential\\ \\
$S$ & Spacing potential\\ \\
$V$ & Lyapunov potential function\\ \\
$p_\theta$ & Average linear momentum of a group of particles\\ \\
$R$ & Center of mass of a group of particles\\ \\
$\theta_f$ & Final velocity direction of a group of particles\\ \\
$(x_{c0}, y_{c0})$ & Initial center of mass of the group of particles
\end{tabular}
\begin{tabular}{lp{5.0in}}
$\left<x, y\right>$ & Inner product of \textbf{$x$} and \textbf{$y$}\\ \\
$\Gamma$ & Invariant set for circular formation\\ \\
$\Gamma'$ & Invariant set for the synchronized and balanced circular formation\\ \\
$\sigma$ & Weighting parameter between orientation and spacing potential
\end{tabular}




%\begin{tabular}
%$\Delta_{\rm{hop}}$ & Delay associated with each hop a message makes
%over network \\ \\
%$\lambda$ & Tuning parameter for algorithm RCA \\ \\
%$\psi_i$ & Heading of $i^{\text{th}}$ UAV \\ \\
%$\psi_{T_j}$ & Heading of target $T_j$ \\ \\
%$\theta$ & LOS angle \\ \\
%$\omega_{\max}$ & Maximum turn rate of a UAV \\ \\
%$\mathbf{a}_{\rm in}$ & Acceleration for deconfliction in the collision plane \\ \\
%$\mathbf{a}_{\rm out}$ & Acceleration for deconfliction out of the
%collision plane \\ \\
%$a_i$ & Acceleration of $U_i$ \\ \\
%$\mathcal{C}(U_i,T_j)$ & Set
%of UAVs in the coalition formed by
%$U_i$ to prosecute $T_j$ \\ \\
%$\mathcal{D}$ & Destination \\ \\
%$\mathcal{D}(U_i,T_j)$ & Set of distances to $T_j$ of UAVs in  $\mathcal{C}(U_i,T_j)$\\ \\
%$D^{T_j}_{U_i}$ & Roundabout path length from $U_i$ to $T_j$ \\ \\
%$\bar{D}^{T_j}_{U_i}$ & Dubins path length from $U_i$ to $T_j$ \\ \\
%%$d$ & LOS separation \\ \\
%${\rm ETA}_i$ & Estimated time of arrival for $U_i$ \\ \\
%$H_{\rm{max}}$ & Maximum number of hops a message is allowed to
%make
%\\ \\
%$\hat{i},\hat{j}$ & Unit vectors \\ \\
%%$k,K$ & Constant for proportional controller \\ \\
%$M$ & Number of targets \\ \\
%$\mathcal{N}_i$ & Set of neighbors of $U_i$ \\ \\
%$N$ & Number of UAVs \\ \\
%$\mathbf{n}$ & Vector perpendicular to collision plane \\ \\
%$(U_i,T_j)$ & UAVs that responded to
%coalition request of $U_i$ for $T_j$ \\ \\
%\end{tabular}
%
%\begin{tabular}{lp{5.0in}}
%$\mathbf{p}_i$ & Position of $i^\text{th}$ UAV, $\mathbf{p}_i =
%(x_i,y_i,z_i)$ \\ \\
%$Q$ & Dimension of each particle in PSO \\ \\
%${R}^{U_i}$ & Resource capability vector of $U_i$,
%${R}^{U_i}=(R^{U_i}_1,\ldots,R^{U_i}_n)$ \\ \\
%${R}^{T_i}$ & Resource capability vector of $T_i$,
%${R}^{T_i}=(R^{T_i}_1,\ldots,R^{T_i}_m)$ \\ \\
%$R$ & Radius of turn \\ \\
%$R_{\rm comm}$ & Communication range of UAV \\ \\
%$R_{\rm des}$ & Desired radius of turn \\ \\
%$R_{\rm min}$ & Minimum radius of turn \\ \\
%$R_{\rm sen}$ & Sensor radius of UAV \\ \\
%$r$ & LOS separation \\ \\
%$S$ & Swarm size in PSO \\ \\
%$\tau$ & Total time for mission completion \\ \\
%$\tau_c^{T_j}$ & Time taken to prosecute $T_j$ after coalition is formed\\ \\
%$\tau^{T_j}_{U_k}$ & ETA of $U_k$ to $T_j$ \\ \\
%$\tau_{T_j}(P,P')$ & Estimated time taken by target $T_j$ to
%travel from
%point $P$ to point $P'$ \\ \\
%$\tau_{U_i}(P,P')$ & Time taken by $U_i$ to take a roundabout path
%from
%point $P$ to point $P'$ \\ \\
%$\tau_s$ & Search time \\ \\
%$T_j$ & $j^{\rm{th}}$ target \\ \\
%$t$ & time \\ \\
%$t_{\rm go}$ & time to go \\ \\
%$U_i$ & $i^{\text{th}}$ UAV \\ \\
%$V^k_l$ & Velocity of $l^{\textrm{th}}$ particle at
%$k^{\textrm{th}}$ time step in PSO, $V^k_l =
%(v^k_{l_1},v^k_{l_2},\ldots, v^k_{l_Q})$ \\ \\
%$V_{T_j}$ & Velocity of target $T_j$ \\ \\
%$V_i$ & Velocity of $i^{\text{th}}$ UAV \\ \\
%\end{tabular}

%\begin{tabular}{lp{5.0in}}
%
%$V_{\rm max}$ & Upper bound for UAV velocity \\ \\
%$V_{\rm min}$ & Lower bound for UAV velocity \\ \\
%$\mathbf{v}_i$
%& Velocity vector of $i^{\text{th}}$ UAV,
%$\mathbf{v}_i=(u_i,v_i,w_i)$ \\ \\
%$X^k_l$ & Position of $l^{\textrm{th}}$ particle at
%$k^{\textrm{th}}$ time step in PSO, $X^k_l = (x^k_{l_1},
%x^k_{l_2},\ldots,x^k_{l_Q})$ \\ \\
%$(x_i,y_i)$ & Position of $U_i$ \\ \\
%$(x_{T_j},y_{T_j})$ & Position of $T_j$ \\ \\
%%\end{tabbing}
%\end{tabular}

%\vspace{0.5cm}
%\textbf{Abbreviations}\\
%
%\indent
%\begin{tabular}{lp{5.0in}}
%ATC & Air Traffic Control \\ \\
%DoF & Degree of Freedom \\ \\
%ETA & Earliest/Estimated Time of Arrival \\ \\
%%IP & Internet Protocol \\ \\
%LOS & Line of Sight \\ \\
%MAC & Medium Access Control\\ \\
%OCFA& Optimal Coalition Formation Algorithm \\ \\
%PI  & Proportional Integral \\ \\
%PN  & Proportional Navigation \\ \\
%PSO & Particle Swarm Optimization \\ \\
%PTCFA& Polynomial Time Coalition Formation Algorithm \\ \\
%RCA & Reactive Collision Avoidance \\ \\
%SGT & Satisficing Game Theory \\ \\
%TCP & Transmission Control Protocol\\ \\
%TTL & Time to Live \\ \\
%UAV & Unmanned Aerial Vehicle \\ \\
%ZEM & Zero Effort Miss \\ \\
%\end{tabular}

}


==> Preamble/preamble.tex <==
%-------------------------------------------------------------------
%                     Preamble
% Contains
%     1. Abstract
%     2. Acknowledgements
%     3. Table of Contents
%     4. List of Tables
%     5. List of Figures
%     6. Notations
%-----------------------------------------------------------------



\def\thepage{\hspace*{-0.5in}\roman{page}}
\begingroup
\leftskip=-1.5in


\input{../preamble/abstract.tex}
\cleardoublepage

\input{../preamble/ack.tex}
\cleardoublepage

\batchmode  \tableofcontents \cleardoublepage

%\listoftables
%\cleardoublepage

\listoffigures
\cleardoublepage

%\listofalgorithms
%\cleardoublepage


\input{../preamble/notations.tex}
\cleardoublepage


\endgroup
\setcounter{page}{1}
\def\thepage{\hspace*{-0.5in}\arabic{page}}

